Are Metrics Enough? Guidelines for Communicating and Visualizing Predictive Models to Subject Matter Experts

Presenting a predictive model's performance is a communication bottleneck that threatens collaborations between data scientists and subject matter experts. Accuracy and error metrics alone fail to tell the whole story of a model - its risks, strengths, and limitations - making it difficult for subject matter experts to feel confident in their decision to use a model. As a result, models may fail in unexpected ways or go entirely unused, as subject matter experts disregard poorly presented models in favor of familiar, yet arguably substandard methods. In this paper, we describe an iterative study conducted with both subject matter experts and data scientists to understand the gaps in communication between these two groups. We find that, while the two groups share common goals of understanding the data and predictions of the model, friction can stem from unfamiliar terms, metrics, and visualizations - limiting the transfer of knowledge to SMEs and discouraging clarifying questions being asked during presentations. Based on our findings, we derive a set of communication guidelines that use visualization as a common medium for communicating the strengths and weaknesses of a model. We provide a demonstration of our guidelines in a regression modeling scenario and elicit feedback on their use from subject matter experts. From our demonstration, subject matter experts were more comfortable discussing a model's performance, more aware of the trade-offs for the presented model, and better equipped to assess the model's risks - ultimately informing and contextualizing the model's use beyond text and numbers.

==> contents/sec-abstract.tex <==
%% Abstract version 3
\abstract{
Presenting the complexities of a model's performance is a communication bottleneck that threatens collaborations between data scientists and subject matter experts.
Accuracy and error metrics alone fail to tell the whole story of a model -- its risks, strengths, and limitations -- making it difficult for subject matter experts to feel confident in deciding to use a model.  As a result, models may fail in unexpected ways if their weaknesses are not clearly understood.  Alternatively, models may go unused, as subject matter experts disregard poorly presented models in favor of familiar, yet arguably substandard methods.   
In this paper, we describe an iterative \strike{interview study}{ study} conducted with both subject matter experts and data scientists to understand the gaps in communication between these two groups.
We find that, while the two groups share common goals of understanding the data and predictions of the model, friction can stem from unfamiliar terms, metrics, and visualizations -- limiting the transfer of knowledge to SMEs and discouraging clarifying questions to be asked during presentations.
Based on our findings, we derive a set of communication guidelines that use visualization as a common medium for communicating the strengths and weaknesses of a model.  We provide a demonstration of our guidelines in a regression modeling scenario and elicit feedback on their use from subject matter experts. 
From our demonstration, subject matter experts were more comfortable discussing a model's performance, more aware of the trade-offs for the presented model, and better equipped to assess the model's risks -- ultimately informing and contextualizing the model's adoption.
}

% %% ABSTRACT VERSION 2

% % However, the use of statistical techniques also changes the risk profile of any downstream tasks, due to bias and noise in the model's predictions.  That risk profile must be clearly understood, documented, and communicated across many different stakeholders in a highly regulated environment.  Aggregated performance metrics such as explained variance or mean average error fail to tell the whole story, making it difficult for subject matter experts to feel confident in deciding to use a model.

% \abstract{
% The use of machine learning and AI models has become ubiquitous across organizations large and small.
% %
% In the deployment of these models, data scientists are expected to deliver complex yet interpretable information about a model's performance to a wide range of audiences.
% %
% Despite growing work focusing on how data scientists may best communicate these results to non-technical audiences, empirical research shows that, in practice, data scientists still rely on aggregated metrics to convey the performance of their models. 
% %
% Accuracy and error metrics alone fail to tell the whole story of a model -- its risks, strengths, and limitations -- making it difficult for subject matter experts to feel confident in deciding to use a model.
% %
% As a result, predictive models frequently go unused, as subject matter experts disregard poorly presented models in favor of familiar, yet arguably substandard methods -- suggesting a mismatch in visual communication research and applied practice.
% %
% In this paper, we examine the impact of visualization and visual communication on model interpretation beyond commonly used performance metrics.
% %
% Using regression as a baseline for our research, we conduct an interview study with 7 data scientists and 6 subject matter experts who frequently collaborate on the development of predictive models. 
% %
% Through a quantitative and qualitative analysis of our interviews, we highlight common communication barriers that exist between the two groups, including language differences and unmet model visualization needs. 
% %
% We then distill a set of visualization guidelines that can assist data scientists who must present the nuances of a model's performance to subject matter experts.
% %
% To evaluate the efficacy of our proposed guidelines, we conduct a second interview study with subject matter experts who offer feedback on the appropriateness of each guideline for both interpreting and making decisions around machine learning models.
% %
% Our results suggest that the use of our guidelines in a presentation of a model's performance enhances the comfort and confidence for subject matter experts, leading to a higher adoption of models used in practice.
% }

% %% ABSTRACT VERSION 1
% % \abstract{
% % The collaborative development of machine learning models has become standard practice across model builders and consumers at both small and large organizations. 
% % %
% % At the heart of these collaborations is a communication workflow requiring data scientists to interface with multiple subject matter experts before a model can be approved for use.
% % % 
% % Often, the success of a model's deployment is dependent on the data scientist's ability to deliver complex yet interpretable information about a model's strengths and weaknesses.
% % %
% % The onus of both building \textit{and} communicating the results of a machine learning model is often left to the data scientist, with recent guidance focusing on presenting to an audience that is either highly technical (i.e., other data scientists) or non-technical (i.e., traditional stakeholders). 
% % %
% % In this paper, we study how visualization and visual communication can aid in the interpretability of a model's capabilities beyond standard performance metrics.
% % %
% % Using regression as a baseline for our research, we conduct an interview study with 7 data scientists and 6 subject matter experts who frequently collaborate on the development of machine learning models. 
% % %
% % Through a quantitative and qualitative analysis of our interviews, we highlight common communication frictions that exist between the two groups. We then distill a set of visualization guidelines that can assist data scientists who must present the nuances of a model's performance to subject matter experts.
% % %
% % To evaluate the efficacy of our proposed guidelines, we conduct a second interview study with subject matter experts who offer feedback on the appropriateness of each guideline for both interpreting and making decisions around a machine learning model.
% % %
% % Our results show that the use of our guidelines in a presentation of a model's performance enhances the comfort and confidence of subject matter experts who must use the model.
% % }


% % sentence 1: background
% % sentence 2: missing gap (e.g. "however, there's a problem blah")
% % sentence 3: why is this bad
% % sentence 4: "In this paper, we propose SystemX"
% % sentence 5, 6 (and/or 7): technical depth on what SystemX is. That is, what is the secret sauce that makes SystemX possible?
% % sentence 8: benefits of SystemX, aka the primary contribution of the paper (note that this should echo sentence 3 in that SystemX should have addressed the problem stated in sentence 3)
% % sentence 9: "We evaluate SystemX..."
% % sentence 10: "Our results indicate that (probelm stated in sentence 3 is no longer a problem)..."


% % Call to research – why understanding this space is different from current visualization research. Visual communication is necessary for data scientists (the speaker) who must present to an audience. Our community should consider how we help this workflow

% %%% VAHC abstract
% % Statistical regression methods can help pharmaceutical organizations improve the quality of their pharmacovigilance by predicting the expected quantity of adverse events during a trial.  However, the use of statistical techniques also changes the risk profile of any downstream tasks, due to bias and noise in the model's predictions.  That risk profile must be clearly understood, documented, and communicated across many different stakeholders in a highly regulated environment.  Aggregated performance metrics such as explained variance or mean average error fail to tell the whole story, making it difficult for subject matter experts to feel confident in deciding to use a model.  In this work, we describe guidelines for communicating regression model performance for models deployed in predicting adverse events.  First, we describe an interview study in which both data scientists and subject matter experts within a pharmaceutical organization describe their challenges in communicating and understanding regression performance.  Based on the responses in this study, we develop guidelines for which visualizations to use to communicate performance, and use a publicly available trial safety database to demonstrate their use.

==> contents/sec-limitations.tex <==
\section{Limitations}
\label{sec:limitations}

\subsection{Scope of Our Interview Study}

The requirements gathered during our study represent only a subset of people working with regression model interpretability in practice. Therefore, the scope of our requirement gathering is narrowed to both the high funding received towards data science and ML/AI, and the high familiarity of data science by interview participants. Our interviews were conducted at a large corporation that employs over X workers, with dedicated departments that employ experts in data science and artificial intelligence. Moreover, our interviewees are highly educated professionals (metric about their education) who are considered experts in their field of study. (Talk about participants being in and outside of US?)

Additionally, our interview study did not attempt to quantify whether the challenges faced by our data scientists and subject matter experts are common across a variety of domains, skill levels, and corporations. In prior literature, studies have been done to understand industry practices across a multitude of domains~\cite{hong2020human}, in addition to sectors outside of `Big Tech'~\cite{hopkins2021machine}. Instead, our study aims to characterize \textit{how} regression model performance is assessed and communicated (e.g., presentation styles, language used, metrics, visualizations). 

\subsection{Scope of the Problem}

In this paper we focus on regression model performance communication, as opposed to general machine learning interpretability. While it is possible that the methods suggested by our framework could be mapped to any predictive model, we did not ask interview participants any questions unrelated to regression models specifically. Therefore, 

==> contents/sec-validation.tex <==
% \begin{table*}[ht!]
%     \centering
%     % \small 
%     \renewcommand{\arraystretch}{1.9}
%     \centering
%     \scalebox{0.9}{
%     \input{tabulars/results}}
%     \caption{
%     Table illustrating a mapping of our guidelines to an actual data science presentation, shown to SMEs in the follow-up study described in Section~\ref{sec:validation}. 
%     % We demonstrate an application of our guidelines with four proposed visualizations (\textbf{V1}-\textbf{V4}) and supplementary model performance information (\textbf{D1}-\textbf{D4}). 
%     % Table illustrating our proposed guidelines and visualizations evaluated in the 2nd scenario of our validation study with SMEs (Section~\ref{sec:validation}). 
%     Each row represents a presentation element (\textbf{V1}-\textbf{V4} and \textbf{D1}-\textbf{D4}) that was shown to SMEs during a PowerPoint presentation of two models' performance (KNN vs. XGB). The left column shows the guideline(s) that are represented, the middle column describes how the guideline(s) are addressed, and the right column includes SMEs' feedback for the guidelines. For the visualizations shown in the middle column, the chart on the left depicts KNN and the right depicts XGB. SMEs rated the effectiveness of each presentation element on a Likert scale of 1 (lowest) to 7 (highest) -- more details on the questionnaire in Section~\ref{sec:protocol}.}
%     \label{tab:validation_results_guideline}
% \end{table*}

% \begin{table}[t!]
%     \centering
%     % \renewcommand{\arraystretch}{1.2}
%     \resizebox{.9\linewidth}{!}{%
%     \input{tabulars/validation-by-pid}}
%     \caption{Results of our validation study described in Section~\ref{sec:validation}.}
%     \label{tab:validation_results_model}
% \end{table}

\section{Demonstration of the Guidelines}
\label{sec:validation}
 
We demonstrate the use of our guidelines in an actual data science presentation through a follow-up interview with SMEs. For this demonstration, we developed two slide-based presentations on distinct regression modeling scenarios: the first presentation without our guidelines, and the second presentation with the use of our guidelines.
Our demonstration includes four types of annotated visualizations to illustrate the model's performance, as well as supplementary information for the model such as data descriptors, terminology definitions, and objective-driven examples of the model performing both well and poorly.

We then shared both presentations with four SMEs in a second round of interviews, treating the first presentation as a ``typical data science presentation'', and the second as an experimental presentation. During this follow-up, we elicited feedback on the effectiveness of the visualizations and communication methods (\textit{i.e.}, guidelines) used in the second presentation.  For the remainder of the section, we first explain our choices of visualizations and how they relate to our guidelines, and finally describe the feedback received from SMEs.
% } 

\subsection{Presentation Elements}
The presentations given to SMEs for our demonstration walked through distinct regression modeling scenarios. Both scenarios describe a new model being proposed (XGB\cite{chen2016xgboost}) to replace the current baseline model in use (KNN\cite{fix1989knn}). A description of both scenarios and the prediction tasks are provided in Section~\ref{sec:protocol}. Note that each scenario uses a unique dataset with a unique prediction task: the first presentation (without guidelines) presented a regression task on the Auto MPG dataset\cite{donoho1982autompg}, while the second presentation (with our guidelines) presented a regression task on the California Housing dataset\cite{pace1997calihousing}.  
Our primary goal for setting up our follow-up study in this manner was to elicit feedback from SMEs on how our guidelines and visualizations could be helpful (or not helpful) in interpreting a new model being proposed, using a standard data science presentation as a point of comparison. 

\subsubsection{Model Performance Visualizations}
We employed four different visualizations, based on our guidelines, to illustrate differences in performance for the two models. Every visualization for XGB (the new model) included a comparison visualization to KNN (the baseline model) (\hlgVis{G2}). For each visualization, one or more annotations were included (\hlgVis{G1}) in our slides to point to specific outliers (\hlgLimit{G4}), differences (\hlgContext{G8}), and conclusions (\hlgContext{G9}) between the two models. 
Full versions of the visualizations can be seen in Table~\ref{tab:validation_results_guideline}, and all source code is provided in an Observable notebook\footnote{\url{https://observablehq.com/@anon1234/model-comm-vis}}. The visualizations used in our follow-up are described as follows: \\

\noindent 
\textbf{(V1) Heatmap by error category and feature distribution: } 

\begin{wrapfigure}{l}{0.1\textwidth}
    \centering
    \includegraphics[width=0.1\textwidth]{figures/teaser/cali_knn_heatmap_small.pdf}
    \includegraphics[width=0.1\textwidth]{figures/teaser/cali_knn_fdp.pdf}
\end{wrapfigure}

\noindent 
A heatmap that illustrates aggregate errors (y-axis) across a single feature (x-axis), using a distinct color scale for each row. The heatmap can help SMEs see how different aggregate measures (\hlgVis{G3}) differ across groups (\hlgLimit{G4}) and determine if a model's performance has weaknesses along the selected feature (\hlgLimit{G6}). This is especially important when looking at how a model performs across regions of data, making sure that a model with a slight increase in overall accuracy does not sacrifice performance within a specific group. Attached to the heatmap is a one-dimensional scatterplot showing the distribution of the feature used to create the grouping, to allow for viewing individual instances when interpreting aggregate measures. \\

\noindent 
\textbf{(V2) Correlation scatterplot with confidence ellipse:}  

\begin{wrapfigure}{l}{0.1\textwidth}
    \centering
    \includegraphics[width=0.1\textwidth]{figures/teaser/cali_knn_corr_sp.pdf}
\end{wrapfigure}

\noindent 
A scatterplot with predicted values from the model plotted on the x-axis, and actual values plotted on the y-axis. Behind the plotted points is a 95\% confidence interval (or covariance ellipse\cite{covarianceEllipse}) that serves as a graphical proxy for the regression metric R2\cite{friendly2013elliptical} (\hlgVis{G3}).  By simultaneously displaying the aggregate metric R2 along with individual instances in the scatterplot, it provides a visual interpretation for the R2 metric.  In addition, it makes it easy to see outliers in predictions and labels (\hlgLimit{G4}). \\

\noindent
\textbf{(V3) Histogram for predicted values versus actual values:}

\begin{wrapfigure}{l}{0.1\textwidth}
    \centering
    \includegraphics[width=0.1\textwidth, height=.96cm]{figures/teaser/cali_xgb_histogram_pred_newcolors.pdf}
    \includegraphics[width=0.1\textwidth, height=.96cm,]{figures/teaser/cali_xgb_histogram_act_newcolors.pdf}
\end{wrapfigure}

\noindent 
Two 1-dimensional histograms, each showing the distributions of a model's prediction and actual values, respectively (\hlgLimit{G5}).  By highlighting the differences in shape of predicted versus actuals, this visualization makes it easy to see if a model might have biases (\textit{i.e.}, missing the high-range outliers found in the ground truth, or missing one of the modes of the distribution of actual values) (\hlgLimit{G4}). \\

\noindent 
\textbf{(V4) Bar chart with global error:}  

\begin{wrapfigure}{l}{0.1\textwidth}
    \centering
    \includegraphics[width=0.1\textwidth]{figures/teaser/cali_knn_bar_global.pdf}
\end{wrapfigure}

\noindent 
A bar chart where each bar represents the absolute error of a single instance; bars are sorted by descending error.  This chart shows the \textit{shape} of error by the models, and conveys how it apportions error, whether by apportioning it equally among all instances, or confining it to few (\hlgLimit{G6}).   A red horizontal line is added to represent the mean absolute error, giving more context to the per instance error for the MAE and MSE metrics. (\hlgVis{G3})

\subsubsection{Supplemental Model Information}
In addition to the four visualizations described above, we also included supplementary information in the second modeling scenario of the presentation given to SMEs. This supplementary information was designed to reflect the guidelines described in Section~\ref{sec:guidelines}; how each maps to our guidelines is described in Table~\ref{tab:validation_results_guideline}.  In total, there were four differences (\textbf{D1}-\textbf{D4}) incorporated into the presentation of our second scenario. The additional information was embedded and highlighted in our presented slides, and can be found in our supplemental material. We briefly describe each below: 

\begin{itemize}[topsep=2pt, partopsep=2pt,itemsep=2pt,parsep=2pt]
    \item[\textbf{D1}] { \textbf{Asking for clarification:} An initial slide that encouraged SMEs to stop us at any time to ask clarifying questions. (\hlgContext{G7})}
    
    \item[\textbf{D2}] { \textbf{Detailing the data:} A table that defined each attribute (or feature) used for training and testing the XGB and KNN models. (\hlgLimit{G5})}
    
    \item[\textbf{D3}] { \textbf{Defining all terminology:} High-level descriptions of the modeling algorithms (KNN and XGB) and how they differ in deriving their predictions. Definitions for R2, MSE, and MAE were supplied. These definitions included how a lower or higher value for each metric translate to relative performance. (\hlgContext{G8})}
    
    \item[\textbf{D4}] { \textbf{Highlighting model weaknesses:} Several examples of XGB performing worse than KNN, on both instance-levels and visualized regions of data. Each example included: (1) a short description to explain why we believed XGB was predicting worse than KNN for these specific examples, and (2) how this performance would relate to real-world objectives (\hlgLimit{G6}, \hlgContext{G9}).}
\end{itemize}

\subsection{Participants \& Protocol}
\label{sec:protocol}
Approximately six months after the original interview study, the six SMEs who participated were contacted for a follow-up interview, with four agreeing to participate.
Our second round of interviews were held virtually in a one-on-one one-hour session.  Each session began with a reminder of their previous participation in the study, and then proceeded through two sets of slides describing the two modeling scenarios (Auto MPG with no guidelines; California Housing with our guidelines).  All of our presented slides are available as supplemental material.
 
\begin{itemize}[leftmargin=0pt,topsep=4pt, partopsep=0pt,itemsep=2pt,parsep=2pt]

    \item[] {\textbf{Follow-up questions:} 
    At the end of the second presentation, SMEs were asked to evaluate the effectiveness for each of the visualizations used (\textbf{V1}-\textbf{V5}) and individual presentation differences between the first and second presentation (\textbf{D1}-\textbf{D4}). For each visualization and individual difference, SMEs rated their agreement to the following statement:
    \begin{itemize}[leftmargin=4pt,topsep=2pt, partopsep=0pt,itemsep=2pt,parsep=2pt]
        \item[] { ``\textit{I found this visualization / difference to be helpful in interpreting the model’s performance.}''}
    \end{itemize}
    Agreement was made on a 7-point Likert scale of 1 (Strongly Disagree) to 7 (Strongly Agree). SMEs also gave open-ended feedback about which aspects of the second presentation (with guidelines) they found helpful when compared to the first presentation (without guidelines).}

\end{itemize}

\subsection{SME Feedback}
We present the results of our follow-up questionnaire as well as the general qualitative feedback from SMEs on the use of our guidelines in a data science presentation. We refer to the participating SMEs in our follow-up study using their original PIDs from Section~\ref{sec:interviews} (see Table~\ref{tab:interview_demographics}). The results for all follow-up questions can be found in Table~\ref{tab:validation_results_guideline}.
% Then, we assess our hypothesis that providing more information about the model performance results in more confidence in decision making.  Lastly, we present general qualitative feedback that came out of the experiment.
% \remco{sugggestion: break the results into more categories (than 3). See below for my suggestion on how to break up the first finding. The last finding on VIS can also be separated into ``VIS is good'' and ``Offline (interactive) VIS is even better''}
% \smallbreak
% \noindent 

\subsubsection{Learning Outcomes: Using Visualization}
The helpfulness of our visualizations were rated on a Likert scale of 1 (lowest) to 7 (highest). \textbf{V1 - Heatmap} (7.0), \textbf{V2 - Scatterplot} (6.5), and \textbf{V3 - Histogram} (6.0) were all considered helpful for interpreting the models' performance, while \textbf{V4 - Bar chart} (2.75) was not considered helpful. Ratings can also be seen in the right column of Table~\ref{tab:validation_results_guideline}. 
% \dylan{I would cut the whole itemized list below. } 
Below, we discuss the qualitative feedback received from SMEs on each visualization shown in our presentation.

\begin{itemize}[leftmargin=0pt, topsep=2pt, partopsep=2pt,itemsep=2pt,parsep=2pt]
    \item[] { 
    \textbf{A heatmap can easily highlight which regions of the data causes the model to perform best and worst}: 
        The heatmap was considered strongly helpful in interpreting the model's performance by all SMEs, partly due to its easy interpretation (``\textit{Easily interpretable since the colors pop out, colors are easier to draw conclusions from and find outliers. (PID9)}''; ``\textit{I can immediately see which model is better versus which is worse. (PID6)''}), and partly because it communicated the strengths and weaknesses of the model: ``\textit{This one gives you even more detail as to how the models are behaving, where they're having the most errors. (PID7)}''  Although PID12 agreed that the heatmap was strongly helpful in interpreting model performance, they also told us heatmaps can be confusing, and that more time is needed to interpret their color scale: ``\textit{I don't like heatmaps\ldots  I need to have done it myself, because unless I know the colors by heart, it's not that easy to interpret.}''
    }
    
    \item[] {
        \textbf{The bounding ellipse of a correlation scatterplot can immediately alert SMEs of potential outliers}: 
        The scatter plot was found to be useful for understanding the metric R2, as PID12 noted that the ellipse helped them see the difference in precision for the two models (``\textit{With the ellipse in the middle, it was easy to gauge where each model was better}''). It was also helpful for identifying outliers and alerting possible risks by PID6: ``\textit{I immediately see the outliers. It helps assess the overall impact and risk that I would have.}'', and PID7: ``\textit{I can see visually where the difference was, the outliers -- the values falling outside of the ellipse on the left side.}'' PID9 noted that they would like more time to understand the chart: ``\textit{Feels like I could draw a conclusion from it\ldots but I would probably need more time.}''
    }
    
    \item[] {
        \textbf{Comparing distributions with histograms helps assess error, but lacks story-telling flash}:  
        The histogram of predicted versus actuals was considered the easiest visualization to grasp (``\textit{What's really positive is it's very easy to understand. (PID12)}''; ``\textit{It does give a quick reality check in terms of the actual vs. predicted. (PID6)}''), and helped SMEs see what types of errors the two models had (``\textit{Easy to compare the two [predicted vs. actuals) side by side. (PID9)}''). PID7 remarked that the shape of the distributions helped easily assess model error, but did not find it overall useful: ``\textit{It's quite visual, but I didn't somehow find it as useful as the others.}''
    }
    
    \item[] {
        \textbf{\ashley{Change title and possibly text to reinforce that visualizations should tell a clear story}Even with different global error lines, charts with indistinguishable shapes lack conclusive evidence for a model's performance}: 
        Ratings for the bar chart with a global error line ranged from neutral to strongly unhelpful, with all participants remarking that the chart did not seem visually distinguishable between the two models (``\textit{You would need to have it bigger, much bigger to see the differences. (PID12)''}), and so it was not clear what the chart was trying to communicate (``\textit{The shape of the curves are similar, it's just not jumping out at me what conclusion I'm supposed to take from it. (PID9)}'').  However, it was noted by PID7 that, for a different scenario, the chart could be helpful if the distribution of errors was very different: ``\textit{Overall shape was the same and the absolute errors were close.  Probably wasn't as useful in the exercise. But there are probably circumstances where it might be helpful as a more differentiating figure.}''
    }
\end{itemize}

All SMEs provided positive feedback on the use of visualizations to communicate model performance rather than simple text or metrics.  SMEs pointed out that with the supplied visualizations, they had ``\textit{quick}" or ``\textit{instant}" insights into model performance, whereas text or numbers had to be studied.  
Annotated examples in the visualizations (\textbf{\hlgnine{G1}}) were also recounted by SMEs as particularly helpful.

PID9 and PID12 both noted that aside from the instant insights or annotations, they wanted to be able to pore over the visualizations outside of presentations to fully digest all of the information:
% \remco{when I read this I wasn't thinking of a pre-read document, but an interactive vis?}
% SMEs supported the usefulness of providing a pre-read document (\hlgeight{G8}) containing the visualizations shown in our presentation, with PID9 noting:
``\textit{I'm often someone who doesn't react to something initially on a screen\ldots And when it's on the screen and I'm listening to someone present I'm back and forth between listening to the person talking and then looking at the slide\ldots I'm not digesting the visuals. (PID9)}" SMEs supported the usefulness of providing a pre-read document (\hlgeight{G8}) containing the visualizations shown in our presentation.  We believe this also highlights the need for more interactive tools, we discuss this further in Section~\ref{sec:modalities}.  

We conclude that presentations should only include visualizations that tell a clear story: \textbf{V4} was rated considerably lower than all other visualizations due to SMEs' inability to draw a conclusion from it. A pre-read document can also be provided with a more exhaustive collection of visualizations and data, to ensure that the SME is able to ultimately decide for themselves what is relevant and what is not.  
% First, the identification of ``interesting patterns" that would qualify a visualization for the presentation may require subject matter expertise, so the data scientist may make mistakes in assuming what is interesting to the subject matter experts.  Making all visualizations available in an off-line format mitigates this risk.  Second, seeing ``uninteresting" visualizations as part of a deep dive into the model performance can provide more confidence for how ``interesting" the selected views are.

\subsubsection{Learning Outcomes: Extra Model Information} 
% Participant helpfulness ratings for \textbf{D1-D4} and visualizations \textbf{V1-V4} are available in Table~\ref{tab:validation_results_guideline}.  
% \dylan{Can we call this Learning Outcomes: Non-visual presentation styles.  Since the visualizations should also follow from the guidelines.}
In general, all supplemental information for the models (\textbf{D1}-\textbf{D4}) were considered helpful by SMEs, which is not surprising on its own: contextual information is generally helpful during model communication,
% (\hlgContext{G7}-\hlgContext{G9}), 
as evidenced by challenges C6 and C7 from Section~\ref{sec:findings}, and previous work on improving model adoption by SMEs\cite{shah2019making}. 
% \gabe{Do we need a citation for information is generally always helpful?} 
Ranked by average helpfulness score, \textbf{D4 - Highlighting model weaknesses} (6.75) was most helpful, reflecting our finding that understanding the strengths and weaknesses of a model (\hlgLimit{G6}), as well as seeing objective-driven examples of its predictions (\hlgContext{G9}), impacts and informs decision-making.  It was followed by \textbf{D2 - Detailing the data} (6.5) and \textbf{D3 - Defining all terminology} (6.25), which provide additional context on the raw data, the models, and the metrics used in a presentation (\hlgLimit{G5}).  The lowest rated difference \textbf{D1 - Asking for clarification} (5.5) was split, with two SMEs rating it as not helpful or unhelpful, and two SMEs rating it as strongly helpful. 

\begin{itemize}[leftmargin=0pt, topsep=2pt, partopsep=2pt,itemsep=2pt,parsep=2pt]
    \item[] { \textbf{Highlighting the model's weaknesses informs decision-making and provides credibility:} SMEs strongly preferred examples of the model performing poorly, reflecting our previous findings that SMEs need transparency from data scientists on a model's weaknesses (``\textit{It helped me come to the conclusion about whether there's a real performance difference between the two models. (PID7)}''). Similar to the challenge C3 identified in Section~\ref{sec:findings}, PID6 told us that seeing the model's limitations would help him decide whether the model could be improved, or would be a no-go for future tasks: ``\textit{Explanations around why KNN shows such worse results than XGB\ldots  That would help us try to see if it's a valid reason, or if it's a straight no-go and we cannot consider the model.}''
	PID6 also noted that grouping or clustering examples of a model performing worse (with a ``plot'') could be more helpful than showing individual examples: ``\textit{It would make sense to get the complete details for all the data\ldots Like, for these types of houses, this model works the best.  But for these other houses, it doesn't work as well.}'' 
% 	PID9 told us that the use cases provided would require more time to digest: ``\textit{I'd want to dig through the numbers more, especially if it's the first time [receiving the presentation], I would need you to walk me through it.}''
    }
    
    \item[] { \textbf{Describing the data used in training ``beyond numbers'' level-sets the presentation:} 
    SMEs found that detailed descriptions and examples of the data used for modeling provided essential context beyond standard summary statistics (``\textit{Always show this [data descriptors] before you see the numbers. Otherwise they're just numbers. (PID9)}''; ``\textit{The units are different for each of the attributes, so it's helpful to have the explanation. (PID7)}''). PID6 also remarked that being presented on the data helped ground the model and its performance: ``\textit{These [data descriptions] will help everyone [SMEs] be on the same page as the data scientists.  This is what we mean when we mention setting a good stage.}'' PID12 remarked that one slide explaining the data was not enough, and he would need ``\textit{more time to analyze everything.}'' In this case, a pre-read document may be helpful (\hlgeight{G8}) to further detail the data.
    }
    
    \item[] { \textbf{Defining data science terminology, model differences, and error metrics establishes a common framework:} 
    Overall, SMEs found our definitions and descriptions of the models used (KNN and XGB) to be helpful, but to varying degrees. PID7 told us, ``\textit{Without your descriptions, KNN versus XGB could be anything. General information is helpful.}'' On the other hand, PID9 felt less clear on the differences, but still indicated a basic understanding of the models: ``\textit{It's still a bit greek to me. The explanation kind of tells me the new model is likely to be better -- it looks more robust from the description. But I still only have a relative framing rather than a deep understanding.}'' Both PID7 and PID9 suggested that walking through examples with ``named attributes'' in a ``nontechnical context'' could be even more helpful (\hlgeight{G8}). 
    
    Regarding the provided definitions for error metrics, SMEs found them to be helpful, even when already familiar with them: ``\textit{I already know about these [R2, MSE, etc.], what's good and bad. But of course knowing what high versus low error means is helpful. (PID9)}'' Similar to our previous finding C1 in Section~\ref{sec:findings}, SMEs found descriptions for the upper and lower error bounds helped contextualize the model's performance: ``\textit{I don't use R2 or MSE or any of these on a day to day basis. In our world, we use p-values\ldots It's difficult at times to know in which scenarios lower is better or higher is better. (PID7)}'' 
    }
    
    \item[] { \textbf{Encouraging SMEs to ask for clarification allows the presentation to feel like a conversation:}
    The overall sentiment towards our slide that encouraged clarification questions was split. PID9 told us, ``\textit{I think I'd already be proactive if there was something I didn't understand.}'' On the other hand, PID7 felt the addition made our presentation more conversational: ``\textit{The perception it creates when you have this statement is that it's more of an exchange. Without it, it feels like more of an exam.}'' PID6 related it to having a two-way, as opposed to one-way, presentation: ``\textit{It does give you the liberty that nothing is written in stone, it's not something that's one way.  It's kind of a two-way as you go through [the presentation]\ldots  You're not just saying, this is what we are doing.}'' We believe the additional step by data scientists to remind SMEs that they can always pause the presentation to ask questions will help encourage those who may not otherwise (\hlgeight{G7}). 
    }
\end{itemize}

In every circumstance, SMEs found our additional information about the models, the data used in training, and explanations for why a model performed poorly, to be helpful when comparing models. PID7 explained that ``\textit{a more nuanced presentation can give confidence.}'' PID6 found the additional information helped him assess potential risk: ``[In the second presentation] \textit{I can weigh each of these different parameters against everything and try to take more calculated risk. But with the first presentation, I'm really not sure because I'm just dependent on what limited information is provided and if it clicks, it clicks. If it doesn't, then I'm going to lose everything.}"

As PID6 explained to us -- when there is less clarity, it is better to be able to understand where the models perform well and perform poorly, so that risk can be calculated, rather than taking a leap of faith. This finding demonstrates the value of guidelines \textbf{\hlgfour{G4}, \hlgfour{G5}, \hlgfour{G6}}: weaving outliers, strengths, and weaknesses into the model presentation improves the SME's ability to use their own expertise in their assessment of a model's performance.


% In sum, 
Overall, the feedback received from our demonstration during follow-up interviews was positive. 
We found that  \textbf{D1}-\textbf{D5} were all either helpful or neutral, and provide some evidence that guidelines \hlgfour{G5}, \hlgfour{G6}, \hlgeight{G7}, \hlgeight{G8}, and \hlgeight{G9} can be partially addressed with these easy-to-implement additions. 
% Overall, the feedback received from our demonstration during follow-up interviews was positive. 
SMEs generally found the guideline-improved presentation to be helpful enough that the guidelines have been implemented within their institution. We discuss the institutional impact of our guidelines in Section~\ref{sec:novartis}, and limitations of this follow-up study in Section~\ref{sec:limitations}.
%


% PID6: ``[In scenario two] \textit{I can weigh each of these different parameters against everything and try to take more calculated risk. But with scenario one, I'm really not sure because I'm just dependent on what limited information is provided and if it clicks, it clicks. If it doesn't, then I'm going to lose everything.}"

% PID7 explained, a more nuanced presentation can give confidence.  However, when there is less clarity, it's better to be able to understand where our models perform well and perform poorly, so that risk can be calculated, rather than taking a leap of faith.  This finding demonstrates the value of guidelines \textbf{\hlgfour{G4}, \hlgfour{G5}, \hlgfour{G6}}: weaving outliers, strengths, and weaknesses into the model presentation improves the SME's ability to use their own expertise in their decision-making.

% PID7 was the only participant who chose the baseline model in the first scenario, but switched to the XGB model in the second scenario based on a better understanding of the weaknesses of XGB using the visualizations and individual examples.  They explained how their expertise on the model's downstream usage might dictate their choice of model: ``\textit{I might change my answer if you tell me that the problem we're trying to solve is related to old homes or really high average monthly salaries.}"  Our findings suggest that the presentation of a model can make the model consumer more confident when there is a clear answer, but also less confident when there are nuances to their decision.


% % impact confidence in decision-making both positively and negatively.  
% We argue that this is the desirable effect: when there is clarity in how a model will be deployed, as PID7 explained, a more nuanced presentation can give confidence.  However, when there is less clarity, it's better to be able to understand where our models perform well and perform poorly, so that risk can be calculated, rather than taking a leap of faith.  This finding demonstrates the value of guidelines \textbf{\hlgfour{G4}, \hlgfour{G5}, \hlgfour{G6}}: weaving outliers, strengths, and weaknesses into the model presentation improves the SME's ability to use their own expertise in their decision-making.

% \subsubsection{Visualizations encouraged taking a deeper look before their decision.} 3 out of 4 SMEs chose the new in-development model (XGB) in the first scenario, while 4 out of 4 chose XGB in the second scenario (see Table~\ref{tab:validation_results_model}). While it is encouraging that one participant switched to the more performant model (XGB), it is more interesting that 
% % \remco{This finding suggests that scenario 2, which is developed following our design guideline was able to XXXX (do awesome things).} 
% % However, 
% all 4 SMEs reported less confidence in their decision, and 2 out of 4 reported less confidence in communicating why they had this decision in the second scenario.  This does not support the original hypothesis that our SMEs would have increased confidence in the second scenario.
% % \remco{I suggest separating the ``Yay, our hypothesis is confirmed'' from the ``However, there are bad parts'' into different sub-sections. There should be a clean, clear confirmation that your guidelines are good (before dissecting the positive finding to pieces).}
% % However, the overall preference for XGB over KNN was lower for 3 out of 4 SMEs, and participants had generally lower confidence in their decision for the second scenario. 
% % 3 out of 4 SMEs felt equally confident in communicating why they had made their decision on which model to use for the original prediction task.

% This feedback mimics previous findings in communicating uncertainty to improve transparency in decision-making\cite{joslyn2012uncertainty, arshad2015investigating, leclerc2015cry}. However, it contrasts the findings from Guo et al. that visualizing uncertainty and alternative predictions improved user confidence when making decisions\cite{guo2019visualizing}. We believe that choosing to deploy a model may be a different type of decision than measured in previous literature, where the cost of a false negative (deploying a bad model) is very high.  PID6 explained their perspective: ``[In scenario two] \textit{I can weigh each of these different parameters against everything and try to take more calculated risk. But with scenario one, I'm really not sure because I'm just dependent on what limited information is provided and if it clicks, it clicks. If it doesn't, then I'm going to lose everything.}"

% \gabe{Could do a callback to the intro about improving model adoption somewhere in this paragraph if we want.} PID7 was the only participant who chose the baseline model in the first scenario, but switched to the XGB model in the second scenario based on a better understanding of the weaknesses of XGB using the visualizations and individual examples.  They explained how their expertise on the model's downstream usage might dictate their choice of model: ``\textit{I might change my answer if you tell me that the problem we're trying to solve is related to old homes or really high average monthly salaries.}"  Our findings suggest that the presentation of a model can make the model consumer more confident when there is a clear answer, but also less confident when there are nuances to their decision.
% % impact confidence in decision-making both positively and negatively.  
% We argue that this is the desirable effect: when there is clarity in how a model will be deployed, as PID7 explained, a more nuanced presentation can give confidence.  However, when there is less clarity, it's better to be able to understand where our models perform well and perform poorly, so that risk can be calculated, rather than taking a leap of faith.  This finding demonstrates the value of guidelines \textbf{\hlgfour{G4}, \hlgfour{G5}, \hlgfour{G6}}: weaving outliers, strengths, and weaknesses into the model presentation improves the SME's ability to use their own expertise in their decision-making.

% % When discussing why they had lower confidence in their decisions, SMEs told us the additional information we provided in the second scenario added nuance to their decision-making process. This was largely due to our presentation of the new model's limitations, weaknesses, and edge cases through annotated visualizations. By viewing nuances in performance, our participants were made aware of potential tradeoffs in performance on different regions of the data.  These findings suggest that use of AI and ML models in production could be improved if data scientists are upfront with where the model can fail before its deployment. 

% % These findings, combined with the feedback we received from SMEs, suggest that data scientists can help SMEs make more educated decisions by revealing what is known \textit{and} unknown in a model's performance. 

% % \dylan{This is introducing a confounding factor, we don't need to highlight it here.}The high confidence given by SMEs in the first scenario could also be due to the ordering of our evaluation scenarios. Due to the small number of participants in our study, we decided not to randomize the ordering of presentations. 
% % The general high confidence given by SMEs indicates that the presentation we gave in the baseline condition is close to current practices that SMEs are used to receiving. In our discussions with SMEs at the end of the evaluation, they remarked that they had intially felt more confident using XGB since it seemed like there were few limitations or weaknesses of the model. These findings suggest that use of AI and ML models in production could be improved if data scientists are upfront with where the model can fail before its deployment. 

% % \textbf{Choice of visualizations matters}\dylan{Reference to table, where the ranking of visualizations is given.}\fix{Feedback about visualizations} SMEs disclosed that, at times, the takeaway message from our visualizations were difficult to assess during the presentation. PID\fix{X...} remarked that a pre-read document prepared in advance to explain these visualizations would help alleviate their concerns, then the SME could ask followup questions during the actual presentation. Confusion felt by SMEs during our presentation on the visualizations we used (specifically, \fix{V1...VN}) suggests that visualization is indeed not commonly used for data science presentations. We suggest that these concepts be introduced to SMEs by data scientists at a slow pace (\fix{\textbf{GX}}), and annotations are included to assist in their interpretability. \dylan{An addition to the guidelines: all visualizations should be checked by the data scientist, but only helpful ones for this case should be included in the presentation.  However, this puts great control in the hands of the data scientist to potentially obfuscate flaws in the model (see our results).  This means that all information should be left in "supplemental material".  All participants desired more time with the models after being shown our visualizations.  Two options were offered: a preread, or a second meeting after users have the opportunity to look through the information.  Both were seen as good options, with no clear preference overall.  This could be the place for interactive visualizations to help, as well.}

% % \smallbreak 

%%% THIS WAS FROM THE START OF 6 
% \dylan{Here, I think we want to talk more about the visualizations and the presentation style.  Maybe we skip right to 6.2, second scenario.  Then, describe the protocol, but in about half the space.  Then, go to 6.3.}

% \dylan{move or remove}In an effort to recreate a realistic industry scenario, we presented the performance of different regression models using our guidelines and asked SMEs a series of interview questions at the end of the presentation. These questions asked SMEs: (1) to make a decision about the models' usage for a prediction task, (2) for their high-level takeaways from our presentation, and (3) for feedback on the guidelines and visualizations used in our presentation. 

% \dylan{move}In addition to demonstrating our guidelines in an actual data science presentation, we also had the goal of understanding which guidelines the SMEs found to be most and least helpful in assessing a model's performance. Based on the SMEs' feedback, we discuss learning outcomes from the use of our proposed guidelines and how this follow-up study can be extended to further validate our work.

% \subsection{Goals}
% \ashley{Should we get rid of this as a subsection and only include the first goal as part of the last paragraph?}
% In addition to demonstrating our guidelines in an actual data science presentation, we also had the goal of understanding which guidelines the SMEs found to be most and least helpful to assessing a model's performance. Based on our SMEs' feedback, we discuss learning outcomes from the use of our proposed guidelines and how this follow-up study can be extended to further validate our work.
% Our follow-up study had two goals.  First, we wanted to understand which guidelines were most helpful and get feedback on the visualizations that followed our guidelines.  Second, we hypothesized that providing more information on model performance would increase confidence in the decision-making process, based on previous findings that communicating uncertainty improved transparency in various decision-making tasks\cite{joslyn2012uncertainty, arshad2015investigating, leclerc2015cry, guo2019visualizing}. 

==> tabulars/validation-by-pid.tex <==

\begin{tabular}{@{}lcccc@{}}
\toprule
 &
   &
   &
   &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}I am confident in\\ communicating\\ my decision\end{tabular}}} \\
 &
   &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Which model \\ would you use$?$ \end{tabular}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}I am confident \\ in my decision\end{tabular}}} &
   \\
\textbf{PID}        & \textbf{Scenario}  &                &   &   \\ \midrule
\multirow{2}{*}{6}  & Auto MPG           & Definitely XGB & 7 & 7 \\
                    & California Housing & Possibly XGB   & 5 & 4 \\ \midrule
\multirow{2}{*}{7}  & Auto MPG           & Possibly KNN   & 7 & 6 \\
                    & California Housing & Possibly XGB   & 6 & 6 \\ \midrule
\multirow{2}{*}{9}  & Auto MPG           & Probably XGB   & 7 & 7 \\
                    & California Housing & Probably XGB   & 6 & 7 \\ \midrule
\multirow{2}{*}{12} & Auto MPG           & Probably XGB   & 5 & 5 \\
                    & California Housing & Probably XGB   & 4 & 5 \\ \bottomrule
\end{tabular}

==> tabulars/validation-by-scenario.tex <==

\begin{tabular}{@{}ccccc@{}}
\toprule
 &
   &
   &
   &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}I am confident in\\ communicating\\ my decision\end{tabular}}} \\
 &
  \textbf{} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Which model \\ would you use\end{tabular}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}I am confident \\ in my decision\end{tabular}}} &
   \\
\textbf{Scenario}                                                             & \textbf{PID} &                &   &   \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Auto\\ MPG\end{tabular}}           & 6            & Definitely XGB & 7 & 7 \\
                                                                              & 7            & Possibly KNN   & 7 & 6 \\
                                                                              & 9            & Probably XGB   & 7 & 7 \\
                                                                              & 12           & Probably XGB   & 5 & 5 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}California\\ Housing\end{tabular}} & 6            & Possibly XGB   & 5 & 4 \\
                                                                              & 7            & Possibly XGB   & 6 & 6 \\
                                                                              & 9            & Probably XGB   & 6 & 7 \\
                                                                              & 12           & Probably XGB   & 4 & 5 \\ \bottomrule
\end{tabular}
